Interrogating the Explanatory Power of Attention in Neural Machine Translation

Attention models have become a crucial component in neural machine translation (NMT). They are often implicitly or explicitly used to justify the model's decision in generating a specific token but it has not yet been rigorously established to what extent attention is a reliable source of information in NMT. To evaluate the explanatory power of attention for NMT, we examine the possibility of yielding the same prediction but with counterfactual attention models that modify crucial aspects of the trained attention model. Using these counterfactual attention mechanisms we assess the extent to which they still preserve the generation of function and content words in the translation process. Compared to a state of the art attention model, our counterfactual attention models produce 68% of function words and 21% of content words in our German-English dataset. Our experiments demonstrate that attention models by themselves cannot reliably explain the decisions made by a NMT model.

==> edits.tex <==

An important observation in Table \ref{table:contradictory_attention_methods} is that the proposed methods are considerably more effective in preserving function words compared to content words. We attribute this observation to the intuition that the production of function words rely more on the target context, in contrast to content words which rely more on the source context. Accordingly, perturbation in the original attention weights likely has significantly more impact on diminishing content words compared to function words. This intuition also ties well with the main idea behind context gates in which the influence of source context and target context is controlled dynamically \cite{tu2017}. Since the generation of function words relies more on the target context, one can ask to what extent attention is needed for preserving function words? To answer this question, we completely zero out the attention using the ZeroOut method. Row 1 in Table \ref{table:special_attentions} shows that only 9\% of function words were preserved in this method. Moreover it can be seen that the model could not preserve any content word when this method is employed. Interestingly, we found that the preserved function words in this method were all occurrences of ",". Apparently the decoder's language model is so strong in predicting "," without attention. This finding suggests that a basic representation of the source context is still necessary to preserve function words.
